How Can Size and Ceiling Bounds Affect the Complexity of Nonuniform Automata Families?

In the past literature, families of two-way finite automata and pushdown automata having limited state complexity (i.e., the total number of inner states) and stack-state complexity (i.e., the total number of inner states multiplied by the total number of strings "pushable" to a stack), have been studied in direct connection to (mainstream) space-bounded complexity classes equipped with Karp-Lipton style advice of limited size when all inputs given to the automata have bounded length. Here, we acknowledge two major factors -- size and ceiling -- of such families, which have a significant impact on the complexity of finite and pushdown automata families, where the "size" refers to (stack-)state complexity and the "ceiling" refers to an input's length bound. In this line of study, we further explore those effects caused by different sizes and ceilings.

==> eptcsdata.tex <==
\providecommand{\firstpage}{105}
\providecommand{\publicationstatus}{C. C\^{a}mpeanu, M. Kutrib, S. Lombardy (Eds.) \\
Non-Classical Models of Automata and Applications (NCMA 2026)\\
EPTCS 446, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.446.7}{10.4204/EPTCS.446.7}}
\pdfoutput=1

